Recursive one-way Navier Stokes equations with PSE-like cost

Spatial marching methods, in which the flow state is spatially evolved in the downstream direction, can be used to produce low-cost models of flows containing a slowly varying direction, such as mixing layers, jets, and boundary layers. The parabolized stability equations (PSE) are popular due to their extremely low cost but can only capture a single instability mode; all other modes are damped or distorted by regularization methods required to stabilize the spatial march, precluding PSE from properly capturing non-modal behavior, acoustics, and interactions between multiple instability mechanisms. The one-way Navier-Stokes (OWNS) equations properly retain all downstream-traveling modes at a cost that is a fraction of that of global methods but still one to two orders of magnitude higher than PSE. In this paper, we introduce a new variant of OWNS whose cost, both in terms of CPU time and memory requirements, approaches that of PSE while still properly capturing the contributions of all downstream-traveling modes. The method is formulated in terms of a projection operator that eliminates upstream-traveling modes. Unlike previous OWNS variants, the action of this operator on a vector can be efficiently approximated using a series of equations that can be solved recursively, i.e., successively one after the next, rather than as a coupled set. In addition to highlighting the improved cost scaling of our method, we derive explicit error expressions and elucidate the relationship with previous OWNS variants. The properties, efficiency, and accuracy of our method are demonstrated for both free-shear and wall-bounded flows.

==> Picture/Final/HB_Comparison_Fc1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{11}{11}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA (d)}%
\psfrag{016}[cl][cl]{\matlabtextA (c)}%
\psfrag{019}[cl][cl]{\matlabtextA (b)}%
\psfrag{020}[cl][cl]{\matlabtextA (a)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{015}[tc][tc]{\matlabtextB $Re(\alpha)$}%
\psfrag{017}[tc][tc]{\matlabtextB $Re(\alpha)$}%
\psfrag{018}[bc][bc]{\matlabtextB $Im(\alpha)$}%
\psfrag{021}[bc][bc]{\matlabtextB $Im(\alpha)$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 0.5$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $\matlabfragNegXTick 0.5$}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
\psfrag{005}[ct][ct]{\matlabtextC $0.5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $-0.5$}%
\psfrag{007}[rc][rc]{\matlabtextC $-0.25$}%
\psfrag{008}[rc][rc]{\matlabtextC $0$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.25$}%
\psfrag{010}[rc][rc]{\matlabtextC $-0.5$}%
\psfrag{011}[rc][rc]{\matlabtextC $-0.25$}%
\psfrag{012}[rc][rc]{\matlabtextC $0$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.25$}%
%
%% </ytick>

==> Picture/Final/HB_Comparison_solutions1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA (b)}%
\psfrag{019}[cl][cl]{\matlabtextA (a)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[tc][tc]{\matlabtextB $Re_x$}%
\psfrag{018}[bc][bc]{\matlabtextB $Re_y$}%
\psfrag{020}[bc][bc]{\matlabtextB $Re_y$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $400$}%
\psfrag{001}[ct][ct]{\matlabtextC $800$}%
\psfrag{002}[ct][ct]{\matlabtextC $1200$}%
\psfrag{003}[ct][ct]{\matlabtextC $1600$}%
\psfrag{004}[ct][ct]{\matlabtextC $2000$}%
\psfrag{005}[ct][ct]{\matlabtextC $2400$}%
\psfrag{006}[ct][ct]{\matlabtextC $2800$}%
\psfrag{007}[ct][ct]{\matlabtextC $3200$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextC $0$}%
\psfrag{009}[rc][rc]{\matlabtextC $400$}%
\psfrag{010}[rc][rc]{\matlabtextC $800$}%
\psfrag{011}[rc][rc]{\matlabtextC $1200$}%
\psfrag{012}[rc][rc]{\matlabtextC $0$}%
\psfrag{013}[rc][rc]{\matlabtextC $400$}%
\psfrag{014}[rc][rc]{\matlabtextC $800$}%
\psfrag{015}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Picture/Final/HB_Comparison_solutions2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{11}{11}\selectfont\strut}%
\psfrag{013}[cl][cl]{\matlabtextA (b)}%
\psfrag{016}[cl][cl]{\matlabtextA (a)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{014}[tc][tc]{\matlabtextB $R$}%
\psfrag{015}[bc][bc]{\matlabtextB $Y$}%
\psfrag{017}[bc][bc]{\matlabtextB $Y$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $400$}%
\psfrag{001}[ct][ct]{\matlabtextC $600$}%
\psfrag{002}[ct][ct]{\matlabtextC $800$}%
\psfrag{003}[ct][ct]{\matlabtextC $1000$}%
\psfrag{004}[ct][ct]{\matlabtextC $1200$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1200$}%
\psfrag{009}[rc][rc]{\matlabtextC $0$}%
\psfrag{010}[rc][rc]{\matlabtextC $400$}%
\psfrag{011}[rc][rc]{\matlabtextC $800$}%
\psfrag{012}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Picture/Final/HB_Comparison_solutions3.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA (b)}%
\psfrag{023}[cl][cl]{\matlabtextA (a)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[tc][tc]{\matlabtextB $Re_x$}%
\psfrag{022}[bc][bc]{\matlabtextB Pressure}%
\psfrag{024}[bc][bc]{\matlabtextB Pressure}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $400$}%
\psfrag{001}[ct][ct]{\matlabtextC $800$}%
\psfrag{002}[ct][ct]{\matlabtextC $1200$}%
\psfrag{003}[ct][ct]{\matlabtextC $1600$}%
\psfrag{004}[ct][ct]{\matlabtextC $2000$}%
\psfrag{005}[ct][ct]{\matlabtextC $2400$}%
\psfrag{006}[ct][ct]{\matlabtextC $2800$}%
\psfrag{007}[ct][ct]{\matlabtextC $3200$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{008}[bc][bc]{\matlabtextC $\times10^{-3}$}%
\psfrag{014}[bc][bc]{\matlabtextC $\times10^{-2}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextC $-6$}%
\psfrag{010}[rc][rc]{\matlabtextC $-3$}%
\psfrag{011}[rc][rc]{\matlabtextC $0$}%
\psfrag{012}[rc][rc]{\matlabtextC $3$}%
\psfrag{013}[rc][rc]{\matlabtextC $6$}%
\psfrag{015}[rc][rc]{\matlabtextC $-6$}%
\psfrag{016}[rc][rc]{\matlabtextC $-3$}%
\psfrag{017}[rc][rc]{\matlabtextC $0$}%
\psfrag{018}[rc][rc]{\matlabtextC $3$}%
\psfrag{019}[rc][rc]{\matlabtextC $6$}%
%
%% </ytick>

==> Picture/Final/HB_Comparison_solutions4.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA (b)}%
\psfrag{017}[cl][cl]{\matlabtextA (a)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{015}[tc][tc]{\matlabtextB $x^{*}(m)$}%
\psfrag{016}[bc][bc]{\matlabtextB $|p|$}%
\psfrag{018}[bc][bc]{\matlabtextB $|p|$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.05$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.1$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.15$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.2$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{005}[bc][bc]{\matlabtextC $\times10^{-3}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $0$}%
\psfrag{007}[rc][rc]{\matlabtextC $1$}%
\psfrag{008}[rc][rc]{\matlabtextC $2$}%
\psfrag{009}[rc][rc]{\matlabtextC $3$}%
\psfrag{010}[rc][rc]{\matlabtextC $0$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{012}[rc][rc]{\matlabtextC $1$}%
\psfrag{013}[rc][rc]{\matlabtextC $1.5$}%
%
%% </ytick>

==> Picture/Final/TJ_Comparison_Fc1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{024}[cl][cl]{\matlabtextA (d)}%
\psfrag{026}[cl][cl]{\matlabtextA (c)}%
\psfrag{029}[cl][cl]{\matlabtextA (b)}%
\psfrag{030}[cl][cl]{\matlabtextA (a)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{025}[tc][tc]{\matlabtextB $Re(\alpha)$}%
\psfrag{027}[tc][tc]{\matlabtextB $Re(\alpha)$}%
\psfrag{028}[bc][bc]{\matlabtextB $Im(\alpha)$}%
\psfrag{031}[bc][bc]{\matlabtextB $Im(\alpha)$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $5$}%
\psfrag{004}[ct][ct]{\matlabtextC $10$}%
\psfrag{005}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{006}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{007}[ct][ct]{\matlabtextC $0$}%
\psfrag{008}[ct][ct]{\matlabtextC $5$}%
\psfrag{009}[ct][ct]{\matlabtextC $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $-15$}%
\psfrag{011}[rc][rc]{\matlabtextC $-10$}%
\psfrag{012}[rc][rc]{\matlabtextC $-5$}%
\psfrag{013}[rc][rc]{\matlabtextC $0$}%
\psfrag{014}[rc][rc]{\matlabtextC $5$}%
\psfrag{015}[rc][rc]{\matlabtextC $10$}%
\psfrag{016}[rc][rc]{\matlabtextC $15$}%
\psfrag{017}[rc][rc]{\matlabtextC $-15$}%
\psfrag{018}[rc][rc]{\matlabtextC $-10$}%
\psfrag{019}[rc][rc]{\matlabtextC $-5$}%
\psfrag{020}[rc][rc]{\matlabtextC $0$}%
\psfrag{021}[rc][rc]{\matlabtextC $5$}%
\psfrag{022}[rc][rc]{\matlabtextC $10$}%
\psfrag{023}[rc][rc]{\matlabtextC $15$}%
%
%% </ytick>

==> Picture/Final/TJ_Comparison_solutions.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA (d)}%
\psfrag{020}[cl][cl]{\matlabtextA (c)}%
\psfrag{023}[cl][cl]{\matlabtextA (b)}%
\psfrag{024}[cl][cl]{\matlabtextA (a)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[tc][tc]{\matlabtextB $x/D$}%
\psfrag{021}[tc][tc]{\matlabtextB $x/D$}%
\psfrag{022}[bc][bc]{\matlabtextB $r/D$}%
\psfrag{025}[bc][bc]{\matlabtextB $r/D$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $5$}%
\psfrag{002}[ct][ct]{\matlabtextC $10$}%
\psfrag{003}[ct][ct]{\matlabtextC $15$}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $25$}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $5$}%
\psfrag{008}[ct][ct]{\matlabtextC $10$}%
\psfrag{009}[ct][ct]{\matlabtextC $15$}%
\psfrag{010}[ct][ct]{\matlabtextC $20$}%
\psfrag{011}[ct][ct]{\matlabtextC $25$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{012}[rc][rc]{\matlabtextC $0$}%
\psfrag{013}[rc][rc]{\matlabtextC $5$}%
\psfrag{014}[rc][rc]{\matlabtextC $10$}%
\psfrag{015}[rc][rc]{\matlabtextC $0$}%
\psfrag{016}[rc][rc]{\matlabtextC $5$}%
\psfrag{017}[rc][rc]{\matlabtextC $10$}%
%
%% </ytick>

==> Picture/Final/TJ_Comparison_solutions2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{025}[cl][cl]{\matlabtextA (b)}%
\psfrag{028}[cl][cl]{\matlabtextA (a)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{026}[tc][tc]{\matlabtextB $x/D$}%
\psfrag{027}[bc][bc]{\matlabtextB p}%
\psfrag{029}[bc][bc]{\matlabtextB p}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $5$}%
\psfrag{002}[ct][ct]{\matlabtextC $10$}%
\psfrag{003}[ct][ct]{\matlabtextC $15$}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $25$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{006}[bc][bc]{\matlabtextC $\times10^{-3}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $-3$}%
\psfrag{008}[rc][rc]{\matlabtextC $-2$}%
\psfrag{009}[rc][rc]{\matlabtextC $-1$}%
\psfrag{010}[rc][rc]{\matlabtextC $0$}%
\psfrag{011}[rc][rc]{\matlabtextC $1$}%
\psfrag{012}[rc][rc]{\matlabtextC $2$}%
\psfrag{013}[rc][rc]{\matlabtextC $3$}%
\psfrag{014}[rc][rc]{\matlabtextC $-1$}%
\psfrag{015}[rc][rc]{\matlabtextC $-0.8$}%
\psfrag{016}[rc][rc]{\matlabtextC $-0.6$}%
\psfrag{017}[rc][rc]{\matlabtextC $-0.4$}%
\psfrag{018}[rc][rc]{\matlabtextC $-0.2$}%
\psfrag{019}[rc][rc]{\matlabtextC $0$}%
\psfrag{020}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{021}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{022}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{023}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{024}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> Picture/Final/TJ_time_cost.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{028}[cl][cl]{\matlabtextA (b)}%
\psfrag{034}[cl][cl]{\matlabtextA (a)}%
%
\providecommand\matlabtextB{\color[rgb]{1.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{031}[cl][cl]{\matlabtextB $N_{\beta}^{1.0}$}%
%
\providecommand\matlabtextC{\color[rgb]{0.000,1.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{026}[cl][cl]{\matlabtextC $N_{\beta}^{1.2}$}%
\psfrag{032}[cl][cl]{\matlabtextC $N_{\beta}^{1.4}$}%
%
\providecommand\matlabtextD{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{029}[tc][tc]{\matlabtextD $N_{\beta}$}%
\psfrag{030}[bc][bc]{\matlabtextD Memory cost (MB)}%
\psfrag{035}[tc][tc]{\matlabtextD $N_{\beta}$}%
\psfrag{036}[bc][bc]{\matlabtextD Wall time/step (s)}%
%
\providecommand\matlabtextE{\color[rgb]{1.000,0.000,1.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{027}[cl][cl]{\matlabtextE $N_{\beta}^{1.4}$}%
\psfrag{033}[cl][cl]{\matlabtextE $N_{\beta}^{1.5}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextF{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextF $15$}%
\psfrag{001}[ct][ct]{\matlabtextF $20$}%
\psfrag{002}[ct][ct]{\matlabtextF $25$}%
\psfrag{003}[ct][ct]{\matlabtextF $30$}%
\psfrag{004}[ct][ct]{\matlabtextF $35$}%
\psfrag{005}[ct][ct]{\matlabtextF $40$}%
\psfrag{006}[ct][ct]{\matlabtextF $45$}%
\psfrag{007}[ct][ct]{\matlabtextF $50$}%
\psfrag{013}[ct][ct]{\matlabtextF $15$}%
\psfrag{014}[ct][ct]{\matlabtextF $20$}%
\psfrag{015}[ct][ct]{\matlabtextF $25$}%
\psfrag{016}[ct][ct]{\matlabtextF $30$}%
\psfrag{017}[ct][ct]{\matlabtextF $35$}%
\psfrag{018}[ct][ct]{\matlabtextF $40$}%
\psfrag{019}[ct][ct]{\matlabtextF $45$}%
\psfrag{020}[ct][ct]{\matlabtextF $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextF 10^{0}}%
\psfrag{009}[rc][rc]{\matlabtextF 10^{1}}%
\psfrag{010}[rc][rc]{\matlabtextF 10^{2}}%
\psfrag{011}[rc][rc]{\matlabtextF 10^{3}}%
\psfrag{012}[rc][rc]{\matlabtextF 10^{4}}%
\psfrag{021}[rc][rc]{\matlabtextF 10^{-2}}%
\psfrag{022}[rc][rc]{\matlabtextF 10^{-1}}%
\psfrag{023}[rc][rc]{\matlabtextF 10^{0}}%
\psfrag{024}[rc][rc]{\matlabtextF 10^{1}}%
\psfrag{025}[rc][rc]{\matlabtextF 10^{2}}%
%
%% </ytick>

==> Picture/Final/WF_Comparison_F.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA (d)}%
\psfrag{022}[cl][cl]{\matlabtextA (c)}%
\psfrag{025}[cl][cl]{\matlabtextA (b)}%
\psfrag{026}[cl][cl]{\matlabtextA (a)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[tc][tc]{\matlabtextB $Re(E_{N_{\beta}})$}%
\psfrag{023}[tc][tc]{\matlabtextB $Re(E_{N_{\beta}})$}%
\psfrag{024}[bc][bc]{\matlabtextB $Im(E_{N_{\beta}})$}%
\psfrag{027}[bc][bc]{\matlabtextB $Im(E_{N_{\beta}})$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 0.5$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextC $\matlabfragNegXTick 0.5$}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{008}[ct][ct]{\matlabtextC $1$}%
\psfrag{009}[ct][ct]{\matlabtextC $1.5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $-1$}%
\psfrag{011}[rc][rc]{\matlabtextC $-0.5$}%
\psfrag{012}[rc][rc]{\matlabtextC $0$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{014}[rc][rc]{\matlabtextC $1$}%
\psfrag{015}[rc][rc]{\matlabtextC $-1$}%
\psfrag{016}[rc][rc]{\matlabtextC $-0.5$}%
\psfrag{017}[rc][rc]{\matlabtextC $0$}%
\psfrag{018}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{019}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> Picture/Final/WF_Comparison_PM.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{024}[cl][cl]{\matlabtextA (d)}%
\psfrag{026}[cl][cl]{\matlabtextA (c)}%
\psfrag{029}[cl][cl]{\matlabtextA (b)}%
\psfrag{030}[cl][cl]{\matlabtextA (a)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{025}[tc][tc]{\matlabtextB $Re(\alpha)$}%
\psfrag{027}[tc][tc]{\matlabtextB $Re(\alpha)$}%
\psfrag{028}[bc][bc]{\matlabtextB $Im(\alpha)$}%
\psfrag{031}[bc][bc]{\matlabtextB $Im(\alpha)$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 8$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 4$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $4$}%
\psfrag{004}[ct][ct]{\matlabtextC $8$}%
\psfrag{005}[ct][ct]{\matlabtextC $\matlabfragNegXTick 8$}%
\psfrag{006}[ct][ct]{\matlabtextC $\matlabfragNegXTick 4$}%
\psfrag{007}[ct][ct]{\matlabtextC $0$}%
\psfrag{008}[ct][ct]{\matlabtextC $4$}%
\psfrag{009}[ct][ct]{\matlabtextC $8$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $-30$}%
\psfrag{011}[rc][rc]{\matlabtextC $-20$}%
\psfrag{012}[rc][rc]{\matlabtextC $-10$}%
\psfrag{013}[rc][rc]{\matlabtextC $0$}%
\psfrag{014}[rc][rc]{\matlabtextC $10$}%
\psfrag{015}[rc][rc]{\matlabtextC $20$}%
\psfrag{016}[rc][rc]{\matlabtextC $30$}%
\psfrag{017}[rc][rc]{\matlabtextC $-30$}%
\psfrag{018}[rc][rc]{\matlabtextC $-20$}%
\psfrag{019}[rc][rc]{\matlabtextC $-10$}%
\psfrag{020}[rc][rc]{\matlabtextC $0$}%
\psfrag{021}[rc][rc]{\matlabtextC $10$}%
\psfrag{022}[rc][rc]{\matlabtextC $20$}%
\psfrag{023}[rc][rc]{\matlabtextC $30$}%
%
%% </ytick>

==> Picture/Final/WF_Comparison_solutions.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA (c)}%
\psfrag{014}[cl][cl]{\matlabtextA (b)}%
\psfrag{016}[cl][cl]{\matlabtextA (a)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{013}[tc][tc]{\matlabtextB $x$}%
\psfrag{015}[tc][tc]{\matlabtextB $x$}%
\psfrag{017}[tc][tc]{\matlabtextB $x$}%
\psfrag{018}[bc][bc]{\matlabtextB $y$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $5$}%
\psfrag{003}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
\psfrag{005}[ct][ct]{\matlabtextC $5$}%
\psfrag{006}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{007}[ct][ct]{\matlabtextC $0$}%
\psfrag{008}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextC $-5$}%
\psfrag{010}[rc][rc]{\matlabtextC $0$}%
\psfrag{011}[rc][rc]{\matlabtextC $5$}%
%
%% </ytick>

==> Picture/Final/WF_E_plot2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[tc][tc]{\matlabtextA $N_{\beta}$}%
\psfrag{010}[bc][bc]{\matlabtextA $error_{k}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB 10^{-4}}%
\psfrag{005}[rc][rc]{\matlabtextB 10^{-3}}%
\psfrag{006}[rc][rc]{\matlabtextB 10^{-2}}%
\psfrag{007}[rc][rc]{\matlabtextB 10^{-1}}%
\psfrag{008}[rc][rc]{\matlabtextB 10^{0}}%
%
%% </ytick>

==> Picture/Final/WF_errorplot.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[tc][tc]{\matlabtextA $N_{\beta}$}%
\psfrag{012}[bc][bc]{\matlabtextA Solution Error}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $6$}%
\psfrag{001}[ct][ct]{\matlabtextB $10$}%
\psfrag{002}[ct][ct]{\matlabtextB $14$}%
\psfrag{003}[ct][ct]{\matlabtextB $18$}%
\psfrag{004}[ct][ct]{\matlabtextB $22$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB 10^{-10}}%
\psfrag{006}[rc][rc]{\matlabtextB 10^{-8}}%
\psfrag{007}[rc][rc]{\matlabtextB 10^{-6}}%
\psfrag{008}[rc][rc]{\matlabtextB 10^{-4}}%
\psfrag{009}[rc][rc]{\matlabtextB 10^{-2}}%
\psfrag{010}[rc][rc]{\matlabtextB 10^{0}}%
%
%% </ytick>

==> Picture/Final/WF_time_cost.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{030}[cl][cl]{\matlabtextA (b)}%
\psfrag{033}[cl][cl]{\matlabtextA (a)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{031}[tc][tc]{\matlabtextB $N_{\beta}$}%
\psfrag{032}[bc][bc]{\matlabtextB Memory cost (MB)}%
\psfrag{034}[tc][tc]{\matlabtextB $N_{\beta}$}%
\psfrag{035}[bc][bc]{\matlabtextB Wall time (s)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $5$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $15$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $25$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
\psfrag{006}[ct][ct]{\matlabtextC $35$}%
\psfrag{007}[ct][ct]{\matlabtextC $40$}%
\psfrag{008}[ct][ct]{\matlabtextC $45$}%
\psfrag{009}[ct][ct]{\matlabtextC $50$}%
\psfrag{015}[ct][ct]{\matlabtextC $5$}%
\psfrag{016}[ct][ct]{\matlabtextC $10$}%
\psfrag{017}[ct][ct]{\matlabtextC $15$}%
\psfrag{018}[ct][ct]{\matlabtextC $20$}%
\psfrag{019}[ct][ct]{\matlabtextC $25$}%
\psfrag{020}[ct][ct]{\matlabtextC $30$}%
\psfrag{021}[ct][ct]{\matlabtextC $35$}%
\psfrag{022}[ct][ct]{\matlabtextC $40$}%
\psfrag{023}[ct][ct]{\matlabtextC $45$}%
\psfrag{024}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC 10^{0}}%
\psfrag{011}[rc][rc]{\matlabtextC 10^{1}}%
\psfrag{012}[rc][rc]{\matlabtextC 10^{2}}%
\psfrag{013}[rc][rc]{\matlabtextC 10^{3}}%
\psfrag{014}[rc][rc]{\matlabtextC 10^{4}}%
\psfrag{025}[rc][rc]{\matlabtextC 10^{0}}%
\psfrag{026}[rc][rc]{\matlabtextC 10^{1}}%
\psfrag{027}[rc][rc]{\matlabtextC 10^{2}}%
\psfrag{028}[rc][rc]{\matlabtextC 10^{3}}%
\psfrag{029}[rc][rc]{\matlabtextC 10^{4}}%
%
%% </ytick>
